Sampling-based Decentralized Monitoring for Networked Embedded Systems

Decentralized monitoring (DM) refers to a monitoring technique, where each component must infer, based on a set of partial observations if the global property is satisfied. Our work is inspired by the theoretical results presented by Baurer and Falcone at FM 2012, where the authors introduced an algorithm for distributing and monitoring LTL formulae, such that satisfaction or violation of specifications can be detected by local monitors alone. However, their work is based on the main assumption that neither the computation nor communication take time, hence it does not take into account how to set a sampling time among the components such that their local traces are consistent. In this work we provide a timed model in UPPAAL and we show a case study on a networked embedded systems board.

==> eptcsdata.tex <==
\providecommand{\firstpage}{85}
\providecommand{\publicationstatus}{Bortolussi, Bujorianu, Pola (Eds.): HAS 2013\\
EPTCS 124, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.124.9}{10.4204/EPTCS.124.9}}
\pdfoutput=1

